Optimizing Latent Space Directions For GAN-based Local Image Editing

Generative Adversarial Network (GAN) based localized image editing can suffer from ambiguity between semantic attributes. We thus present a novel objective function to evaluate the locality of an image edit. By introducing the supervision from a pre-trained segmentation network and optimizing the objective function, our framework, called Locally Effective Latent Space Direction (LELSD), is applicable to any dataset and GAN architecture. Our method is also computationally fast and exhibits a high extent of disentanglement, which allows users to interactively perform a sequence of edits on an image. Our experiments on both GAN-generated and real images qualitatively demonstrate the high quality and advantages of our method.

==> tables/comparison_table.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{graphicx}
\newcommand\RotText[1]{\rotatebox{90}{\parbox{2cm}{\centering#1}}}

\begin{table*}[t]

\resizebox{\textwidth}{!}{%
\begin{tabular}{c|ccccccccl}
% \hline
\begin{tabular}[c]{@{}c@{}}GAN-based Image \\ Editing Algorithms\end{tabular} & 
\begin{tabular}[c]{@{}c@{}}Supervision\end{tabular} &
% Supervision & 
\begin{tabular}[c]{@{}c@{}}Works on\\ any Dataset\end{tabular} &
\begin{tabular}[c]{@{}c@{}}No test-time\\optimization\end{tabular} 
&\begin{tabular}[c]{@{}c@{}}any GAN\\ architecture\end{tabular} & \begin{tabular}[c]{@{}c@{}}Single Image\\ Edit\end{tabular} & \begin{tabular}[c]{@{}c@{}}Global\\ Semantic Edits\end{tabular} & \begin{tabular}[c]{@{}c@{}}Localized\\ Semantic Edits\end{tabular} & 
\begin{tabular}[c]{@{}c@{}}Editing\\ Any Object\end{tabular} & 
\\
\hline \hline
% \cline{1-10}
\cite{GANSpace, UnsupervisedLatentSpaceGAN, ClosedFormFactorization}                                                                      & Unsupervised    & \cmark                                                            & \cmark & \cmark                                                                                                  & \cmark                                                                 & \cmark                                                                   & \xmark                                                                  & \xmark 
% & \parbox[]{2cm}{\multirow{8}{*}{\rotatebox[]{90}{Latent Space Traversal}}} \\
& \multirow{8}{*}{\rotatebox{90}{\parbox{3cm}{\centering \\ \textbf{\hspace{3pt} Latent Space Traversal}}}} \\
\cite{ContinuousFactorVariationGAN, GANSteerability}                                              & Self-Supervised & \cmark                                                            & \cmark & \cmark                                                                                                             & \cmark                                                                 & \cmark                                                                   & \xmark                                                                  & \xmark &                                                                   \\
InterFaceGAN \cite{InterFaceGAN}                                                                 & Supervised      & \xmark                                                             & \cmark  & \cmark                                                                                                           & \cmark                                                                 & \cmark                                                                  & \cmark                                                                  & \xmark &                                                                  \\

GANALYZE \cite{GANalyze}                                                                     & Supervised      & \cmark                                                            & \cmark & \cmark                                                                                               & \cmark                                                                 & \cmark                                                                   & \xmark                                                                  & \xmark  &                                                                 \\
StyleSpace \cite{StyleSpace}                                                                     & Supervised      & \cmark                                                            & \cmark                                                             & \xmark                                                            & \cmark                                                                 & \xmark                                                                   & \cmark                                                                  & \cmark  &                                                                 \\
Zhu et al. \cite{lowrankGAN}                                                                     & Unsupervised      & \cmark                                                   & \xmark                                                               & \cmark                                                            & \cmark                                                                 & \xmark                                                                   & \cmark                                                                  & \xmark  &                                                                 \\
\textbf{LELD (Ours)}                                                                   & Supervised      & \cmark                                                 & \cmark                                                              & \cmark                                                            & \cmark                                                                 & \xmark                                                                  & \cmark                                                                 & \cmark &                                                                   \multirow{8}{*}{\rotatebox{90}{\parbox{3cm}{\centering \textbf{\hspace{0pt} Image Composition}}}} \\
\hline \hline
% \cline{1-10}
Bau et al. \cite{RewritingGAN}                                                      & Unsupervised    & \cmark                                                      & \xmark                                                              & \xmark                                                            & \xmark                                                                  & \xmark                                                                  & \cmark                                                                 & \cmark &  \\
Chai et al. \cite{gan_compositionality}                                                      & Unsupervised    & \cmark                                            & \cmark                                                              & \cmark                                                            & \xmark                                                                  & \xmark                                                                  & \cmark                                                                 & \cmark &                                                                   \\
Editing in Style \cite{EditingInStyleEDO}                                                             & Unsupervised    & \cmark                                             & \cmark                                                               & \xmark                                                             & \xmark                                                                  & \xmark                                                                   & \cmark                                                                 & \xmark  &                                                                  \\
Zhang et al. \cite{decorate_bedroom}                                                  & Supervised      & \xmark                                          & \cmark                                                             & \xmark                                                             & \xmark                                                                  & \xmark                                                                  & \cmark                                                                 & \cmark  &                                                                  \\

Barbershop \cite{BarbershopGI}       & Supervised    & \cmark                                                  & \cmark                                                              & \xmark                                                             & \xmark                                                                  & \xmark                                                                  & \cmark                                                                 & \xmark &                                                                   \\ 


% \hline \hline

% \vspace{10pt}
% \hline
% \hline
\end{tabular}}
\vspace{10pt}
\caption{Comparison of GAN-based Image editing algorithms by category.}
\label{image_edit_comparison}
\end{table*}
